Invariants of a general branched cover of ${\bf P}^{1}$

We investigate the resolution of a general branched cover $\alpha : C \to {\bf P}^1$ in its relative canonical embedding $C \subset {\bf P} E$. We conjecture that the syzygy bundles appearing in the resolution are balanced for a general cover, provided that the genus is sufficiently large compared to the degree. We prove this for the Casnati-Ekedahl bundle, or "bundle of quadrics" $F$ - the first bundle appearing in the resolution of the ideal of the relative canonical embedding. Furthermore, we prove the conjecture for all syzygy bundles in the resolution when the genus satisfies $g = 1 \mod d$.

==> TODO <==
TODO:

- fix figure 2 description.


Later:
- Run spell check (aspell -t -c file.tex) again
- To fine tune position of labels, manually edit argument of \put command in the pdf_tex files.
- If we reexport images with transparency, run:
pdf2ps, ps2pdf to rasterize image, or:
 ps2pdfwr -dCompatibilityLevel=1.4 -r1200 -dHaveTransparency=false transverse-directrices.pdf sanitized.pdf
 to rasterize it.


- P_a vs P_i. What did we decide again?
  Anand: Maybe we can use a bold P for the chain?
  - Ok! I am going through and replacing every ``P_?'' denoting a chain by
    ``\chain{?}''. In the main file I defined \chain{k}=\P_k, but if we change our minds later it should be an one-liner.

- Q: Is there a elliptic fibration with a genus g d-section for every d and g? 

@Misc{bopp_macaulay2_2015,
author =   {Bopp, Christian and Hahn, Michael},
title =    {RelativeCanonicalResolution.m2 -- construction of relative canonical resolutions and Eagon-Northcott type complexes},
howpublished = {\url{http://www.math.uni-sb.de/ag-schreyer/images/data/computeralgebra/M2/doc/Macaulay2/RelativeCanonicalResolution/html/index.html}},
year = {2015}
}
